Game Theory with Simulation of Other Players

Game-theoretic interactions with AI agents could differ from traditional human-human interactions in various ways. One such difference is that it may be possible to simulate an AI agent (for example because its source code is known), which allows others to accurately predict the agent's actions. This could lower the bar for trust and cooperation. In this paper, we formalize games in which one player can simulate another at a cost. We first derive some basic properties of such games and then prove a number of results for them, including: (1) introducing simulation into generic-payoff normal-form games makes them easier to solve; (2) if the only obstacle to cooperation is a lack of trust in the possibly-simulated agent, simulation enables equilibria that improve the outcome for both agents; and however (3) there are settings where introducing simulation results in strictly worse outcomes for both players.

==> author_contributions.tex <==
\section*{Contribution Statement}

While the technical parts of the paper were written down by the first author, all three authors made comparable contributions to the underlying ideas.

% \co{I'm happy with this contribution statement. :-) Do we need it for IJCAI, though? Given space...}
% \vk{My preference would be to drop it for IJCAI but include it in arXiv
%     (both because I endorse contribution statements in general and because Vince's contribution is larger than you would assume by default).}

==> ethical_statement.tex <==
\section*{Ethical Statement}

A possible downside of this research is that the results also apply to the setting where an agent is simulated against their will.
    In case of AI agents, this would correspond to using a stolen source code.
    In case of humans, it would correspond to abusing private data and using machine-learning algorithms to predict behaviour.
    While both of these scenarios are concerning, we believe the present paper does not make this adversarial simulation any easier, and therefore does not make this risk any worse.
\co{Did reviewers ask for this? To me this is a bit random, in part for the reason you mention.}
\vk{My preference would be to drop it for IJCAI but include it in arXiv.
    This is a weak preference though.
    Reasoning: I endorse ethical statements on the grounds that including them by default even when not needed creates a bigger pressure to include them for papers where it is needed.}
\co{Ah, hmm... That's noble, but... I endorse not writing anything when one doesn't have anything interesting to say on the grounds that saying uninteresting stuff strengthens norms of saying uninteresting stuff.}
\vk{Hah. Fair.}
